Intensity-Coupled-Polarization in Instruments with a Continuously Rotating Half-Wave Plate

We discuss a systematic effect associated with measuring polarization with a continuously rotating half-wave plate. The effect was identified with the data from the E and B Experiment (EBEX), which was a balloon-borne instrument designed to measure the polarization of the CMB as well as that from Galactic dust. The data show polarization fraction larger than 10\% while less than 3\% were expected from instrumental polarization. We give evidence that the excess polarization is due to detector non-linearity in the presence of a continuously rotating HWP. The non-linearity couples intensity signals into polarization. We develop a map-based method to remove the excess polarization. Applying this method for the 150 (250) GHz bands data we find that 81\% (92\%) of the excess polarization was removed. Characterization and mitigation of this effect is important for future experiments aiming to measure the CMB B-modes with a continuously rotating HWP.

==> tex/conclusion.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Summary}

Continuously rotating HWP are increasingly used in CMB instruments to measure polarization on large scales as they mitigate low frequency noise and reduce \ac{ICP}
originating from detector differencing. 
Because diameters of HWP are currently limited to a maximum of $\sim 0.5$~m, HWPs often have to be placed behind the mirror and lenses in the 
optical chain of a telescope. This also enables HWPs to be kept at a cold temperature which minimizes load on the detectors. 
However as a result, detectors measure $\ac{ICP}^{IP}$ from the optical elements sky side of the \ac{HWP}, and polarized signals 
from the instrument are modulated by the HWP and dominate the detector time-streams. 
These HWP synchronous signals can push detectors in the non-linear regime and create \ac{ICP}$^{NL}$ along with other non-linear effects such as compression of $I^{sky}$ and $P^{sky}$. 
All sources of ICP create spurious E- and B-modes, and can also create low frequency noise in polarization for ground-based experiments in which the main $I$ source is the atmosphere.

We examined in this paper the excess polarization in EBEX maps and proposed a model for its origin involving a $\sim 10$\% coupling between $I$ and $P$ originating from detector non-linearity
in the presence of a HWPSS of order several hundred fW. We showed that non-linearity can be mitigated by either acting on the detector response or minimizing the HWPSS. 
%We demonstrated that the excess polarization was exactly out of phase with the HWPSS 4th harmonic phase.
We proposed a map-based method to measure the coupling fraction and angle for each detector, which is usable to measure \ac{ICP} from any origin.
We showed that in EBEX 81 (92) \% of the ICP was removed from the CMB at 150 (250) GHz using this technique.
Because future experiments are expected to have much smaller coupling, this map-based method can be used to measure and subtract \ac{ICP} and improve CMB polarization measurements and achievable constraints on $r$.

\section*{Acknowledgement}
\acknowledgments
Didier acknowledges a NASA NESSF fellowship NNX11AL15H.
Support for the development and flight of the EBEX instrument was provided by
NASA grants NNX12AD50G, NNX13AE49G,
NNX08AG40G, and NNG05GE62G, and by NSF grants AST-0705134 and ANT-0944513.
We acknowledge support from the Italian INFN INDARK Initiative.
Ade and Tucker acknowledge the
Science \& Technology Facilities Council for its continued support of the
underpinning technology for filter and waveplate development.
We also acknowledge support by the Canada Space Agency, the Canada
Research Chairs Program, the Natural Sciences and
Engineering Research Council of Canada, the Canadian Institute for Advanced Research,
the Minnesota Supercomputing Institute, the National Energy Research
Scientific Computing Center, the Minnesota and Rhode Island
Space Grant Consortia, our collaborating institutions, and Sigma Xi the
Scientific Research Society.
Baccigalupi acknowledges support from the RADIOFOREGROUNDS
grant of the European Union's Horizon 2020
research and innovation program (COMPET-05-2015, grant agreement number 687312)
and the INDARK INFN Initiative.

Reichborn-Kjennerud acknowledges an NSF Post-Doctoral Fellowship AST-1102774,
and a NASA Graduate Student Research Fellowship. Raach and Zilic
acknowledge support by the Minnesota Space Grant Consortium.
Helson acknowledges NASA NSTRF fellowship NNX11AN35H.
We very much thank Danny Ball and his colleagues at the Columbia
Scientific Balloon Facility for their dedicated support of the EBEX program.
%We are grateful for contributions to the fabrication of optical elements by Enzo Pascale and
%Lorenzo Moncelsi. 



